Reachability-based Trajectory Design via Exact Formulation of Implicit Neural Signed Distance Functions

Generating receding-horizon motion trajectories for autonomous vehicles in real-time while also providing safety guarantees is challenging. This is because a future trajectory needs to be planned before the previously computed trajectory is completely executed. This becomes even more difficult if the trajectory is required to satisfy continuous-time collision-avoidance constraints while accounting for a large number of obstacles. To address these challenges, this paper proposes a novel real-time, receding-horizon motion planning algorithm named REachability-based trajectory Design via Exact Formulation of Implicit NEural signed Distance functions (REDEFINED). REDEFINED first applies offline reachability analysis to compute zonotope-based reachable sets that overapproximate the motion of the ego vehicle. During online planning, REDEFINED leverages zonotope arithmetic to construct a neural implicit representation that computes the exact signed distance between a parameterized swept volume of the ego vehicle and obstacle vehicles. REDEFINED then implements a novel, real-time optimization framework that utilizes the neural network to construct a collision avoidance constraint. REDEFINED is compared to a variety of state-of-the-art techniques and is demonstrated to successfully enable the vehicle to safely navigate through complex environments. Code, data, and video demonstrations can be found at https://roahmlab.github.io/redefined/.

==> algorithms/rdf_alg.tex <==
\begin{algorithm}[t]
\begin{algorithmic}[1]
\State $\{\pzqi\,:\, i \in \Nt\} \leftarrow (q_0,\dot q_0)$ 
\State $\co, \Go \leftarrow O$ 
\State{\bf for} $i = 1:n_t$ %// for each time steps
    \State\hspace{0.2in}{\bf for} $j = 1:n_q$ % for each joint
        \State\hspace{0.4in} $\pzFOjKi \leftarrow \texttt{PZFO}(\pzqi)$ 
        \State\hspace{0.4in} $\pzFOjki \leftarrow \texttt{slice}(\pzFOjKi, k)$ \label{lst:line:fo}
        \State\hspace{0.4in} $\pzFOjkibuf \leftarrow \pzFOjki\oplus Z_O^g$ \label{lst:line:buffered_fo}
    \State\hspace{0.2in}{\bf end for}
\State{\bf end for}
\State{\bf for} $j = 1:n_q$
    \State\hspace{0.2in} $\Pj \leftarrow \conv(\bigcup_{i = 1}^{\nt}\pzFOjkibuf)$ \label{lst:line:conv}
    %\State\hspace{0.2in} $\{(A_j^{(h)},b_j^{(h)})\,:\, h \in \Nhj\} \leftarrow \texttt{polytope}(\mathcal{P}_j)$
    \State\hspace{0.2in} {\bf if} $c_O \in \Pj$ {\bf then}
    % \State\hspace{0.2in} {\bf if} $A_j\,c_O-b_j \leq 0$ {\bf then} // $c_0 \in \mathcal{P}_j$
        %\State\hspace{0.4in} $\Tilde{r}_j \leftarrow \max_{h\in\Nhj}\frac{A_j^{(h)}\,p-b_j^{(h)}}{||A_j^{(h)}||}$ // negative distance 
        \State\hspace{0.4in} $\ardf_j \leftarrow -\dist(\co,\partial\Pj)$ // negative distance 
    \State\hspace{0.2in} {\bf else}
        %\State\hspace{0.4in} $\Tilde{r}_j \leftarrow \texttt{QP}\left(c_O, \{(A_j^{(h)},b_j^{(h)})\,:\, h \in \Nhj\}\right)$ // positive distance
        \State\hspace{0.4in} $\ardf_j \leftarrow \dist(\co,\partial\Pj)$ // positive distance 
    \State\hspace{0.2in} {\bf end if} 
\State{\bf end for}
\State \textbf{Return} $\{\ardf_j\,:\, j \in \Nq\}$
\end{algorithmic}
\caption{\texttt{RDF}$(q_0, \dot q_0, k, O)$}
\label{alg:rdf}
\end{algorithm}

==> sections/05_rdf.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%~~~~~~~~~~~~~~~~~~~~~~~Overview of RDFs
\section{Reachability-based Signed Distance Functions}
\label{sec:RDF}
\jon{We can either 1) place this in the prelim section; 2) combine with Neural net section; 3) remove altogether}
% This section defines the signed distance function between sets. 
% Signed distance functions are used in robotics in a variety of applications including representing collision avoidance constraints. 
This section describes how to extend the signed distance function to a distance function between the forward reachable set of a robot and an obstacle. 
This novel distance function, which we call the reachability-based signed distance function (\methodname{}), was introduced in \cite[]{michaux2023rdf} and  enables us to formulate the collision avoidance problem between a parameterized reachable set and an obstacle as an optimization problem. 

\subsection{Signed Distance Functions}
We begin by defining an unsigned distance function:
\begin{defn}
Given a set $\Omega \subset \mathbb{R}^{\nd}$, the \defemph{distance function} associated with $\Omega$ is defined by
    \begin{equation}
       \dist(x;\Omega) = \min_{y \in \partial\Omega} \|x - y\|.
    \end{equation}
The \defemph{distance between two sets} $\Omega_1, \Omega_2 \subset \mathbb{R}^{\nd}$ is defined by
    \begin{equation}
       \dist(\Omega_1,\Omega_2) = \min_{\substack{x \in \partial\Omega_1 \\ y \in \partial\Omega_2}} \|x - y\|.
    \end{equation}
\end{defn}
\textbf{Notice that this distance function is zero for sets that have non-trivial intersection. 
As a result, this distance function provides limited information for such sets (i.e., it is unclear how much they are intersecting with one another).
To address this limitation, we consider the following definition:}
\begin{defn} Given a subset $\Omega$ of $\mathbb{R}^{\nd}$, the \defemph{signed distance function} $\sdf$ between a point is a map $\sdf: \mathbb{R}^{\nd} \to \mathbb{R}$ defined as
    \begin{equation}
    \sdf(x; \Omega) = 
        \begin{cases}
          \dist(x, \partial\Omega)  & \text{if } x \not \in \Omega \\
          -\dist(x,\partial\Omega) & \text{if } x \in \Omega.
        \end{cases}
\end{equation}
The \defemph{signed distance between two sets} $\Omega_1, \Omega_2 \subset \mathbb{R}^{\nd}$ is defined as
    \begin{equation}
    \sdf(\Omega_1,\Omega_2) = 
        \begin{cases}
          \dist(\Omega_1,\Omega_2)  & \text{if } \Omega_1 \cap \Omega_2 = \emptyset  \\
          -\dist(\Omega_1,\Omega_2) & \text{otherwise}.
        \end{cases}
\end{equation}
\end{defn}
% \begin{itemize}
%     \item Signed distance functions are a common representation in robotics.
%     \item In this section we give a brief overview of signed distance functions and describe some of their notable properties.
%     \item In the context of motion planning the SDF has been used to compute the distance between a single configuration of a robot and a static obstacle \cite[]{XXX}.
%     \item We then introduce the reachability-based distance function, which represents the distance to a swept volume.
% \end{itemize}


\subsection{Reachability-Based Signed Distance Functions}
This subsection describes the reachability-based distance function as the signed distance function associated with the forward reachable set of the ego vehicle.
% The following sections describe how to overapproximate the forward occupancy and distance calculations with zonotopes using reachability analysis.
\begin{defn}\label{def:rdf_point}
The \defemph{reachability-based distance} function associated with the forward occupancy reachable set $\FO$ is a mapping 
defined by
\begin{equation}
    \rdf(x, \FO) = \min_{j \in \Nj} \rdf_j(x;\FO_j)
\end{equation}
where
$\rdf_j$ is the signed distance function associated with the $j^{th}$ forward occupancy $\FO_j$ such that
\begin{equation}
    \rdf_j(x;\FO_j) = \sdf(x;\FO_j).
\end{equation}
The \defemph{reachability-based distance} between an obstacle $O \subset \mathbb{R}^d$ and the robot's forward occupancy reachable set $\FO$ is defined by
\begin{equation}
    \rdf(O, \FO) = \min_{j \in \Nj} \rdf_j(O, \FO_j).
\end{equation}
\end{defn}
One can use this distance function to formulate trajectory optimization problems as we describe next. \jon{This statement is out of place}



==> sections/approach.tex <==
\section{Reachability-based Signed Distance Function}\label{sec:approach}

\subsection{Signed Distance Between Zonotopes}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\columnwidth]{figures/buffer_obstacle.pdf}
    \caption{Illustration of signed distance for convex polytopes. In particular, this works well with zonotopes.\jon{Add labels. Highlight pos/neg distance better.}} 
    \label{fig:zono_sdf}
    \vspace*{-0.2cm}
\end{figure}
In this section we describe how to compute signed distance between two zonotopes, how to represent this function exactly using a ReLU neural network, and how we leverage this novel representation for representing obstacle-avoidance constraints for safe motion planning.

\begin{defn}\label{defn:zono_pentration_depth}
    The \defemph{penetration depth} of $Z_1$ and $Z_2$ in $\R^{\nd}$ is denoted $\pi(Z_1, Z_2)$ and is defined by 
    \begin{equation}
        \pdf(Z_1, Z_2) = \min \{\|t\| :\ \text{int}(Z_1 + t \cap Z_2) = \emptyset, \quad t \in \R^{\nd}\}.
    \end{equation}
\end{defn}


\begin{lem}\label{lem:zono_sdf}
Let $Z_1 = (c_1, G_1)$ and $Z_2 = (c_2, G_2)$ be zonotopes such that $Z_1 \cap Z_2 \neq \emptyset$. 
Then the signed distance between $Z_1$ and $Z_2$ is given by
\begin{equation}
    \sdf(Z_1, Z_2)  = 
        \begin{cases}
          \dist(c_1; Z_{2,buf})  & \text{if } c_1 \not \in Z_{2,buf} \\
          -\pdf(c_1, Z_{2,\text{buf}}) & \text{if } c_1 \in Z_{2,buf}
        \end{cases} .
\end{equation}
\end{lem}
\begin{proof} See \cite{michaux2023rdf}.
\end{proof}

Maybe say something about how this can be solved using a convex optimization program.
But here, we instead compute the distances exactly.


\begin{lem} \label{lem:hyperplane_distance}
We can compute the distance  
\end{lem}
\begin{proof} Let 
\begin{equation}
    h_i(t) = v_1 + s (v_2 - v_1) 
\end{equation}
for $s \in [0,1]$.

The distance between a point and the line segment is
\begin{equation}
    \phi_i(s) = \|h_i(s) - p\|^2
\end{equation}

\begin{equation}
    \hat{s}_i = \frac{(p - v_1)^T(v_2 - v_1)}{(v_2 - v_1)^T (v_2 - v_1)}
\end{equation}

\begin{equation}
    s^{\ast}_i = \min (\max (\hat{s}_i, 0), 1)
\end{equation}
\end{proof}

\begin{thm} \label{thm:exact_sdf}
The distance between two zonotopes can be computed
\end{thm}
\begin{proof}
\end{proof}
Note that we provide a visual illustration of this theorem in Fig. \ref{fig:zono_sdf}.
We use this to build the neural network in the next section
\subsection{Neural Network Architecture}

\begin{thm}
\label{thm:network_bound}
\end{thm}
\begin{proof}
\end{proof}


% Before proving the required result, we prove several intermediate results. 
% \subsection{Signed Distance Between Zonotopes}
% \label{subsec:sdf_zono}

% Here we derive the signed distance between two zonotopes.
% To proceed we first require a condition for determining if two zonotopes are in collision:
% \begin{lem}\label{lem:zono_intersection}
% Let $Z_1 = (c_1, G_1)$ and $Z_2 = (c_2, G_2)$ be zonotopes. Then $Z_1 \cap Z_2 \neq \emptyset$ if and only if $c_1 \in Z_{2,\text{buf}} = (c_2, G_1 \cup G_2)$.
% \end{lem}
% \begin{proof}
% Suppose the intersection of $Z_1$ and $Z_2$ is non-empty. This is equivalent to the existence of $z_1 \in Z_1$ and $z_2 \in Z_2$ such that $z_1 = z_2$. Furthermore, by definition of a zonotope (Defn. \ref{defn:zonotope}), this is equivalent to the existence of coefficients $\beta_1$ and $\beta_2$ such that $z_1 = c_1 + G_1 \beta_1$, $z_2 = c_2 + G_2 \beta_2$, and
% \begin{align}
%     &c_1 + G_1 \beta_1 = c_2 + G_2 \beta_2 \\
%     \iff& c_1 = c_2 + G_2 \beta_2 - G_1 \beta_1 \\
%     \iff& c_1 \in (c_1, G_1 \cup G_2) = Z_{2, \text{buf}}.
% \end{align}
% Thus we have shown that $Z_1 \cap Z_2 \neq \emptyset$ if and only if $c_1 \in (c_1, G_1 \cup G_2) = Z_{2, \text{buf}}$.
% \end{proof}

% Lemma \ref{lem:zono_intersection} can then be used to compute the the positive distance between two non-intersecting zonotopes:
% \begin{lem}\label{lem:zono_positive_distance}
% Let $Z_1 = (c_1, G_1)$ and $Z_2 = (c_2, G_2)$ be non-intersecting zonotopes.
% \begin{align}
%     \dist(Z_1, Z_2) = \dist(c_1; Z_{2,buf})
% \end{align}
% where $Z_{2,\text{buf}} = (c_2, G_1 \cup G_2)$.
% \end{lem}
% \begin{proof}
% Suppose $Z_1$ and $Z_2$ are non-intersecting zonotopes such that $\dist(Z_1, Z_2) = r$ for some $r \in \mathbb{R}^{+}$. That is, there exists $z_1 \in Z_1$ and $z_2 \in Z_2$ such that 
% \begin{align}
%     r &= \|z_1 - z_2\| \\
%     &= \|c_1 + G_1 \beta_1 - (c_2 + G_2 \beta_2) \| \\
%     &= \| c_1 - (c_2 + G_2 \beta_2 = G_1 \beta_1) \| \\
%     &\geq \dist(c_1, (c_2, G_1 \cup G_2)) \\
%     &= \dist(c_1, Z_{2, \text{buf}}).
% \end{align}
% Now suppose $\dist(c_1, Z_{2, \text{buf}}) = r$. Then there exists coefficients $\beta_1$ and $beta_2$ such that
% \begin{align}
%     r &= \|c_1 - (c_2 + G_1 \beta_1 + G_2 \beta_2) \| \\
%     &= \|c_1 - G_1 \beta_1 - (c_2 + G_2 \beta_2) \| \\
%     &= \|z_1 - z_2\| \\
%     &\geq \dist(Z_1, Z_2).
% \end{align}
% Together, these inequalities prove that $\dist(Z_1, Z_2) = \dist(c_1; Z_{2,buf})$.
% \end{proof}
% Let $\text{int}(S)$ denote the interior of a set.
% Before deriving the negative distance we first define the penetration depth  \cite{cameron1986mtd} of two zonotopes:
% \begin{defn}\label{defn:zono_pentration_depth}
%     The \defemph{penetration depth} of $Z_1$ and $Z_2$ in $\R^{\nd}$ is denoted $\pi(Z_1, Z_2)$ and is defined by 
%     \begin{equation}
%         \pdf(Z_1, Z_2) = \min \{\|t\| :\ \text{int}(Z_1 + t \cap Z_2) = \emptyset, \quad t \in \R^{\nd}\}.
%     \end{equation}
% \end{defn}

% The penetration depth $\pi(Z_1,Z_2)$ can be interpreted as the minimum translation applied to $Z_1$ such that the interior of $Z_1 \cap Z_2$ is empty.
% Following \cite{agarwal2000convex} we can now redefine the penetration distance between $Z_1 = (c_1, G_1)$ and $Z_2 = (c_2, G_2)$ in terms of $c_1$ and $Z_{2,\text{buf}}$.
% \begin{lem}\label{lem:zono_negative_distance}
% Let $Z_1 = (c_1, G_1)$ and $Z_2 = (c_2, G_2)$ be zonotopes such that $Z_1 \cap Z_2 \neq \emptyset$.
% Then the penetration depth between $Z_1$ and $Z_2$ is given by
%    \begin{align}
%      \pdf(Z_1, Z_2) = \pi(c_1, Z_{2,\text{buf}}),
% \end{align} 
% \end{lem}
% \begin{proof}
% Suppose $Z_1 \cap Z_2 \neq \emptyset$. 
% Then by Defn. \ref{defn:zono_pentration_depth}, there exists a translation vector $t \in \R^{\nd}$ such that $\text{int}(Z_1 + t \cap Z_2) = \emptyset$. 
% This means that $Z_1$ is translated by $t$ such that only the boundaries of $Z_1 + t$ and $Z_2$ are intersecting. 
% Thus, there exists $z_1 \in \partial Z_1$ and $z_2 \in \partial Z_2$ such that $z_1 + t = z_2$. 
% Furthermore, there exist coefficients $\beta_1$ and $\beta_2$ such that $z_1 = c_1 + G_1 \beta_1$, $z_2 = c_2 + G_2 \beta_2$, and
% \begin{align}
%     & c_1 + G_1 \beta_1 + t = c_2 + G_2 \beta_2 \\
%     \iff& c_1 + t = c_2 + G_2 \beta_2 - G_1 \beta_1 \in \partial Z_{2,\text{buf}}.
% \end{align}
% Since $\pi(c_1, Z_{2,\text{buf}})$ is the minimum distance between $c_1$ and all points in $\partial Z_{2,\text{buf}}$, this means that $\pi(c_1, Z_{2,\text{buf}}) \leq \|t\|$.

% Now suppose $c_1 \in Z_{2, \text{buf}}$.
% Let $t \in \R^{\nd}$ such that $\|t\|$ is the penetration depth of $c_1$ and $Z_{2,\text{buf}}$. 
% Then there exists coefficients $\beta_1$ and $\beta_2$ such that $z_2 = c_2 + G_1 \beta_1 + G_2 \beta_2$ and
% \begin{align}
%     c_1 + t = c_2 + G_1 \beta_1 + G_2 \beta_2 \\
%     c_1 -G_1 \beta_1 + t = c_2 + G_2 \beta_2.
% \end{align}
% This means translating $z_1 = c_1 - G_1 \beta_1 \in \partial Z_1$ by $t$ causes the boundary of $Z_1$ to intersect the boundary of $Z_2$. 
% Therefore $\pi(Z_1, Z_2) \leq \|t\|$.
% Together the above inequalities prove the result.
% \end{proof}

% \begin{thm}\label{thm:zono_sdf}
% Let $Z_1 = (c_1, G_1)$ and $Z_2 = (c_2, G_2)$ be zonotopes such that $Z_1 \cap Z_2 \neq \emptyset$. 
% % Denote $\mathcal{P} = \bigcap_{i}\mathcal{H}_i$ as the half-space representation of the buffered zonotope $Z_{2,buf} = (c_2, G_1 \cup G_2)$.
% Then the signed distance between $Z_1$ and $Z_2$ is given by
% \begin{equation}
%     \sdf(Z_1, Z_2)  = 
%         \begin{cases}
%           \dist(c_1; Z_{2,buf})  & \text{if } c_1 \not \in Z_{2,buf} \\
%           -\pdf(c_1, Z_{2,\text{buf}}) & \text{if } c_1 \in Z_{2,buf}
%         \end{cases} .
% \end{equation}
% \end{thm}
% \begin{proof} The proof follows readily from Lemmas \ref{lem:zono_positive_distance} and \ref{lem:zono_negative_distance}.
% \end{proof}

% Note that we provide a visual illustration of this theorem in Fig. \ref{fig:zono_sdf}.

% \subsection{The Proof}

% We prove the desired result by considering two cases. 
% First assume  $O \cap \FO(q(T;k)) = \emptyset$ for all $t \in T$. 
% Then
% \begin{align}
%     \rdf(O, \FO(q(T;k))) &= \underset{t \in T}{\min}\: \underset{j \in \Nq}{\min}\:  \sdf(O, \FO_j(q(t;k))) \\
%     &\geq \underset{i \in \Nt}{\min}\: \underset{j \in \Nq}{\min}\:  \sdf(O, \pzFOjki) \\
%     % &= \underset{i \in \Nt}{\min}\: \underset{j \in \Nq}{\min}\: \sdf(O, \pzFOjkibuf) \\
%     &= \underset{i \in \Nt}{\min}\: \underset{j \in \Nq}{\min}\: \sdf(\co, \pzFOjkibuf) \\
%     &= \underset{j \in \Nq}{\min}\: \sdf(\co, \bigcup_{i\in\Nt} \pzFOjkibuf) \\
%     &\geq \underset{j \in \Nq}{\min}\: \sdf(\co, \Pj) \\
%     &= \underset{j \in \Nq}{\min}\: \ardf_j(\co, \Pj) \\
%     &= \ardf(\co, \bigcup_{j\in \Nq} \Pj),
% \end{align}
% where the first equality follows from the definition of $\rdf$ in Def. \ref{def:rdf_point}, the second inequality follows from Lemma \ref{lem:pz_FO}, the third equality follows from Lemma \ref{lem:zono_positive_distance}, the fourth inequality by flipping the order of minimization, and the fifth inequality follows from Def. \ref{def:convhull}. 

% Thus $\ardf$ underapproximates the distance between the forward occupancy and the obstacle. 
% If instead $O \cap \FO_j(\q) \neq \emptyset$ for some $t \in T$, replacing $\geq$ with $\leq$ shows that we can overapproximate the penetration distance between an obstacle and the forward occupancy.

% \begin{lem}\label{lem:zono_negative_distance}
% Let $Z_1 = (c_1, G_1)$ and $Z_2 = (c_2, G_2)$ be zonotopes such that $Z_1 \cap Z_2 \neq \emptyset$. Denote $\mathcal{P} = \bigcap_{i}\mathcal{H}_i$ as the half-space representation of the buffered zonotope $Z_{2,buf} = (c_2, G_1 \cup G_2)$. Then the penetration depth of $Z_1$ and $Z_2$ is
%    \begin{align}
%      \pi(Z_1, Z_2) = \underset{i}{\min}\:\dist(c_1, \mathcal{H}_i),
% \end{align} 
% where $\mathcal{P}$ is the polytope representation of $Z_{2,buf} = (c_2, G_1 \cup G_2)$.
% \end{lem}
% \begin{proof}
%     See Appendix.
%     % It is readily apparent that
%     % \begin{align}
%     %     \pi(Z_1, Z_2) = \pi(c_1, Z_{2,buf}).
%     % \end{align}
% \end{proof}


\subsection{Algorithm}
\input{algorithms/redefine_alg}
\begin{itemize}
    \item Will probably want to 
\end{itemize}


==> sections/symbols.tex <==
\section{List of Symbols}
\subsection{Notation}
\begin{itemize}
    \item $A$: denotes a matrix
    \item $\mathcal A$: set notation (capital letters)
    \item $\mathcal A'$: set notation (capital letters)
    \item $a \in \mathcal A$: element of a set
    \item $\alpha\in \R^n$: vector in $\R^n$ \jon{is this used?}
    \item $[\alpha]_i$: $i$-th element of $\alpha$ \jon{is this used?}
    \item $\diag(\alpha)$: diagonal matrix with $\alpha$ on the diag (used to define interval as zonotope)
    \item $B(\alpha, \epsilon)$: Ball of radius $\epsilon$ centered at $\alpha$ (used in assumption 10)
    \item $\beta \in \R^n$: vector in $\R^n$ \jon{also vector of coefficients}
    \item $\sB$ : Set of all bins
    \item $\epsilon$: small number
    \item $\max$: max
    \item $\min$: min
    \item $\N$: natural numbers
    \item $n \in \N$: natural number
    \item $\np \in \N$: dimension of trajectory parameter
    \item $\nut \in \N$: dimension of controller input
    \item $\nzt \in \N$: dimension of ego vehicle state
    \item $\R$: real numbers
    \item $\R^n$: $n$-dimensional reals
    \item $\Rnp$: real numbers
    \item $\Rnut$: real numbers
    \item $\Rnzt$: real numbers
    \item $\relu(z) = \max\{0,z\}$
    \item $\rot$: rotation matrix (used once in definition 5)
    \item $x$: general element of a set
    \item $y$: general element of a set
\end{itemize}

\subsection{Set-based representations and operations}
\begin{itemize}
    \item $A \Z$: matrix multiplied by a zonotope
    \item $\beta_k$: indeterminant coefficient 
    \item $\beta_{\forall}$: indeterminant coefficient vector
    \item $c$: zonotope center
    \item $\co$: obstacle center
    \item $\conv$: convex hull
    \item $\dist$: distance function
    \item $g_i$: ith zonotope generator
    \item $g_{\forall}$: all generators of a zonotope
    \item $G_i$:  ith generator matrix of Matrix zonotope 
    \item $\Int(\alpha, \beta)$: $n$-dimensional box (Used in definition of ego vehicle)
    \item $\oplus$: Minkowski sum
    \item $\Omega$: general set
    \item $\Omega^{c}$: complement of $\Omega$
    \item $\conv(\Omega)$: convex hull of $\Omega$
    \item $\partial \Omega$: boundary of the set $\Omega$
    \item $s$: signed distance function
    \item $\Z = \zonocg{c}{G}$: zonotope with center $c$ and generator matrix $G$
    \item $\Z_1$: generic zonotope
    \item $\Z_2$: generic zonotope
\end{itemize}

\subsection{Ego Vehicle Dynamic Model}
\begin{itemize}
    \item $f$: nonlinear dynamics model
    \item $\heading$: ego vehicle heading
    \item $u(t) \in \R^m$: control input at time $t$
    \item $\W\subset\R^2$: World space
    \item $\sx(t)$ and $\sy(t)$: position of the vehicle in a two dimensional world space
    \item $z(t) = (\sx(t), \sy(t), \heading) \subset \R^n$: the state of the ego vehicle at time $t$
    \item $\dot{z}(t) \subset \R^n$: time derivative of state
\end{itemize}

\subsection{Trajectory Parameterization}
\begin{itemize}
    \item $n_p$: dimension of trajectory parameter
    \item $p$: trajectory parameter
    \item $\P$: space of trajectory parameters
    \item $t$: time
    \item $T := [0,\tf]$: planning horizon
    \item $\tz$: initial time
    \item $\tf$: fixed time duration
    \item $\tplan$: planning time liimit
\end{itemize}

\subsection{Ego Vehicle Occupancy}
\begin{itemize}
    \item $\E\big(t,z_0,p\big)$: ego vehicle forward occupancy
    \item $l$: length of ego vehicle rectangle 
    \item $\mathcal O^{ego}$: rectangle containing the ego vehicle
    \item $w$: width of ego vehicle rectangle
    \item $z_0\in\Z_0\subset\Rnzt$: initial condition and zonotope
\end{itemize}

\subsection{Environment and Sensing}
\begin{itemize}
    \item $\delta$: sensor radius
    \item $k \in \K$: obstacle index and index set
    \item $\Obskt\subset \W$: current notation for obstacle set
    \item $\vegomax$: max speed of ego vehicle
    \item $\vobsmax$: max speed of obstacles
\end{itemize}

\subsection{Theoretical Motion Planning Problem}
\begin{itemize}
    \item: $\cost:\Z_0\times\P \to \R$: user-specified cost function
    \item $\optth$: theoretical optimizatin problem
\end{itemize}

\subsection{Offline Reachability Analysis}
\begin{itemize}
    \item $A_j \in \R^{2 \times \np}$: matrix that transforms $p$ and adds it to $c_j$ during $\T_j$
    \item $c_j$: zonotope center for time interval $\T_j$
    \item $\Delta_t$: positive number that divides $\tf$
    \item $G_j$: zonotope generators for time interval $\T_j$
    \item $\xi_j(z_0,p)$: zonotope containing the ego vehicle footprint during $\T_j$
    \item $j\in \J$: index and time index set
    \item $\T_j$: $j$-th time interval
    \item $\vartheta(j,k)$: zonotope
\end{itemize}

\subsection{Online Optimization}
\begin{itemize}
    \item $\rdf(\xi(z_0,p)$: reachability-based distance function
    \item $\ardf_{NN}(\FOzj\big(z_0,p\big), \Obszjk)$
\end{itemize}

\subsection{Zonotope Vertex Enumeration}
\begin{itemize}
    \item $\mathbf{0}$: vector/matrix of zeros
    \item $\mathbf{1}$: vector/matrix of ones
    \item $\beta$: indeterminate coefficient vector
    \item $\beta_j$: indeterminate coefficient for generator $g_j$
    \item $C$: coefficient matrix
    \item $C(i,j)$: element of coefficient matrix
    \item $m$: number of generators
    \item $2m$: number of vertices
    \item $V = \{v_1, \cdots, v_{2m}\}$: set of vertices
    \item $\conv(V)$: convex hull of $V$
    \item $p \in \conv(V)$:
    \item $\sigma_i = \sigma_i^{+} -\sigma_i^{-}$: non-negative coefficient constraint equation
    \item $\sigma_1, \cdots, \sigma_{2m}$, with $\sum_{i=1}^{2m}$: non-negative coefficients
\end{itemize}

\subsection{Exact Signed Distance Between Zonotopes}
\begin{itemize}
    \item $j \in \J$: index set
    \item $\Oj = \zonocg{\coj}{\Goj}$: "obstacle" zonotope
    \item $\Obs = \bigcup_{j \in \J} \Oj$: union of "obstacle" zonotopes
    \item $\segij$: line segment between vertices $i$ and $j$ 
    \item $\Z = \zonocg{\cz}{\Gz}$: zonotope 
\end{itemize}
\newpage
